Return of EM: Entity-driven Answer Set Expansion for QA Evaluation

Recently, directly using large language models (LLMs) has been shown to be the most reliable method to evaluate QA models. However, it suffers from limited interpretability, high cost, and environmental harm. To address these, we propose to use soft EM with entity-driven answer set expansion. Our approach expands the gold answer set to include diverse surface forms, based on the observation that the surface forms often follow particular patterns depending on the entity type. The experimental results show that our method outperforms traditional evaluation methods by a large margin. Moreover, the reliability of our evaluation method is comparable to that of LLM-based ones, while offering the benefits of high interpretability and reduced environmental harm.

==> table/ent_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{3}{c}{NQ} & \multicolumn{3}{c}{TQ} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{Numeric} &
  \multicolumn{1}{c}{Non-numeric} &
  \multicolumn{1}{c}{N/A} &
  \multicolumn{1}{c}{Numeric} &
  \multicolumn{1}{c}{Non-numeric} &
  \multicolumn{1}{c}{N/A} \\ \hline
% Insteval                                     & 84.9   & \textbf{90.8}  & \textbf{84.3}  & 91.3   & \textbf{96.2}  & \textbf{92.1}  \\ \hline
Original                                     & 82.6   & 88.1  & 74.7  & 81.2   & 88.2  & 80.1  \\
Freebase                                         & 82.3   & 89.7  & 74.4  & 84.7   & 90.4  & 80.0  \\ \hline
Inst-zero                                  & 82.2   & 84.4  & 74.7  & 84.4   & 90.1  & 79.3  \\
Inst-random                                & 85.9   & 88.0  & 76.8  & 83.5   & 90.8  & 83.9  \\
\textbf{Ours (Inst-Entity)}                                & \textbf{89.3}   & \textbf{90.4}  & \textbf{79.0}  & \textbf{92.4}   & \textbf{93.6}  & \textbf{85.7}  \\ \hline
\end{tabular}%
}
\caption{Average accuracy against human labels across five QA models, using different answer set expansion methods. We separately report the accuracy based on entity types: Numeric, Non-numeric, and N/A.}
\label{tab:ent_result}
\end{table}




==> table/error_case.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|l}
\cline{1-2}
\multicolumn{1}{|c|}{Entity type} & Format types                                                                                      &  \\ \cline{1-2}
\multicolumn{1}{|l|}{\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Numeric\\ - DATE\\ - MONEY\\ - QUANTITY\\ - etc.\end{tabular}}} &
  \begin{tabular}[c]{@{}c@{}}Numerals \\\end{tabular} &
   \\ \cline{2-2}
\multicolumn{1}{|l|}{}           & \begin{tabular}[c]{@{}c@{}}Different representation\\ (symbols, abbreviation, order)\\\end{tabular} &  \\ \cline{2-2}
\multicolumn{1}{|l|}{}           & Specificity                                                                                       &  \\ \cline{2-2}
\multicolumn{1}{|l|}{}           & Unit conversion                                                                                   &  \\ \cline{1-2}
\multicolumn{1}{|l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Non-numeric\\ - PERSON\\ - GPE\\ - ORG\\ - etc.\end{tabular}}} &
  \begin{tabular}[c]{@{}c@{}}Different representation\\ (symbols, abbreviation, order)\\\\\end{tabular} &
   \\ \cline{2-2}
\multicolumn{1}{|l|}{}           & \begin{tabular}[c]{@{}c@{}}\\Specificity\\\\\end{tabular}                                                                                       &  \\ \cline{1-2}
\multicolumn{1}{|l|}{N/A}        & \begin{tabular}[c]{@{}c@{}}Contextual\\ paraphrase\end{tabular}                                   &  \\ \cline{1-2}
\end{tabular}%
}
\caption{}
\label{tab:error_case}
\end{table}





% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|l|}
% \hline
% \multicolumn{1}{|c|}{Entity type} &
%   Format types &
%   Examples \\ \hline
% \multicolumn{1}{|c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\\ \\ \\ \\ Numeric\\- TIME\\- MONEY\\- QUANTITY\\- PERCENT\\- CARDINAL\\- DATE\\- ORDINAL\end{tabular}}} &
%   Numerals &
%   \begin{tabular}[c]{@{}l@{}}
%   % \textbf{[Question]: } what is indian air force rank in the world\\ \textbf{[Gold Answer]: } \textcolor{blue}{fourth}\\ \textbf{[Model Prediction]: } Indian air force rank is \textcolor{red}{4th} in the world.\\ \\
%   \textbf{[Question]: } how many episodes are in season 2 of \\the handmades tale\\ \textbf{[Gold Answer]: } \textcolor{blue}{13}\\ \textbf{[Model Prediction]: } The Season 2 of the Handmaid's Tale \\have \textcolor{red}{thirteen} episodes.\end{tabular} \\ \cline{2-3} 
% \multicolumn{1}{|l|}{} &
%   \begin{tabular}[c]{@{}c@{}}Different\\ representation\\ (symbols,\\ abbreviation,\\ order)\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}
%   % \textbf{[Question]: } how much did the new tappan zee bridge cost\\ \textbf{[Gold Answer]: } \textcolor{blue}{\$3.9 billion}\\ \textbf{[Model Prediction]: } The new Tappan Zee Bridge cost around \\\textcolor{red}{3.9 billion dollars}.\\ \\
%   \textbf{[Question]: } when was ye rishta kya kehlata hai started\\ \textbf{[Gold Answer]: } \textcolor{blue}{January 12, 2009}\\ \textbf{[Model Prediction]: } The Ye Rishta Kya Kehlata Hai\\ started in \textcolor{red}{12, Jan., 2009.}\end{tabular} \\ \cline{2-3} 
% \multicolumn{1}{|l|}{} &
%   Specificity &
%   \begin{tabular}[c]{@{}l@{}}\textbf{[Question]: } what's the population of fargo north dakota\\ \textbf{[Gold Answer]: } \textcolor{blue}{120,762}\\ \textbf{[Model Prediction]: } The population of Fargo, North Dakota \\is \textcolor{red}{about 120,000}.\end{tabular} \\ \cline{2-3} 
% \multicolumn{1}{|l|}{} &
% \begin{tabular}[c]{@{}c@{}}Unit\\Conversion\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}\textbf{[Question]: } how long is the movie son of god\\ \textbf{[Gold Answer]: } \textcolor{blue}{138 minutes}\\ \textbf{[Model Prediction]: } The movie Son of God is \\\textcolor{red}{2 hours and 18 minutes} long.
%   % \\\\ \textbf{[Question]: } How tall was Napoleon?\\ Gold Answer: \textcolor{blue}{168 cm}\\ \textbf{[Model Prediction]: } Napoleon was \textcolor{red}{1.68m} tall.
%   \end{tabular} \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Non-numeric\\- PERSON\\- GPE\\- ORG\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}Different\\ representation\\ (symbols,\\ abbreviation,\\ order)\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}\textbf{[Question]: } where was the ncaa football championship game \\played 2018\\ \textbf{[Gold Answer]: } \textcolor{blue}{Atlanta, Georgia}\\ \textbf{[Model Prediction]: } The 2018 NCAA Football Championship \\Game was played in \textcolor{red}{Atlanta, GA}.\end{tabular} \\ \cline{2-3} 
%  &
%   Specificity &
%   \begin{tabular}[c]{@{}l@{}}\textbf{[Question]: } who ran the fastest 40 time in nfl history\\ \textbf{[Gold Answer]: } \textcolor{blue}{Bo Jackson}\\ \textbf{[Model Prediction]: } The fastest 40 yard dash in NFL history \\was run by \textcolor{red}{Vincent Edward "Bo" Jackson}.\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}N/A\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}
%   Contextual \\paraphrase\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}\textbf{[Question]: } the pectoralis minor is located deep to \\which muscle\\ \textbf{[Gold Answer]: } \textcolor{blue}{beneath the pectoralis major}\\ \textbf{[Model Prediction]: } \textcolor{red}{under the pectoralis major muscle}.\end{tabular} \\ \hline
% \end{tabular}%
% }
% \caption{Categorization of surface form types depending on the entity types. Based on these surface forms, we sample a few-shot examples for each entity type.}
% \label{tab:error_case}
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|l|}
% \hline
% \textbf{Format type} &
%   \textbf{Affected Entity type} &
%   \multicolumn{1}{c|}{\textbf{Example}} \\ \hline
% Numerals &
%   \begin{tabular}[c]{@{}c@{}}TIME\\ MONEY\\ QUANTITY\\ PERCENT\\ CARDINAL\\ DATE\\ ORDINAL\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Question: what is indian air force rank in the world\\ Gold Answer: \textcolor{blue}{fourth}\\ Model Prediction: Indian air force rank is \textcolor{red}{4th} in the world.\\ \\ Question: how many episodes are in season 2 of the \\handmades tale\\ Gold Answer: \textcolor{blue}{13}\\ Model Prediction: The Season 2 of the Handmaid's\\ Tale have \textcolor{red}{thirteen} episodes.\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Different\\ representation\\ (symbols,\\ abbreviation,\\ order)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}TIME\\ MONEY \\ QUANTITY \\ PERCENT \\ DATE \\ GPE \\ ORG\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Question: how much did the new tappan zee bridge cost\\ Gold Answer: \textcolor{blue}{\$3.9 billion}\\ Model Prediction: The new Tappan Zee Bridge cost around \\ \textcolor{red}{3.9 billion dollars}.\\ \\ Question: where was the ncaa football championship game \\played 2018\\ Gold Answer: \textcolor{blue}{Atlanta, Georgia}\\ Model Prediction: The 2018 NCAA Football Championship \\Game was played in \textcolor{red}{Atlanta, GA}.\end{tabular} \\ \hline
% Specificity &
%   \begin{tabular}[c]{@{}c@{}}TIME\\ MONEY\\ QUANTITY\\ PERCENT\\ CARDINAL\\ DATE\\ PERSON\\ GPE\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Question: when was ye rishta kya kehlata hai started\\ Gold Answer: \textcolor{blue}{January 12, 2009}\\ Model Prediction: The Ye Rishta Kya Kehlata Hai started \\ in \textcolor{red}{January, 2009}.\\  
%   % \\ Question: what's the population of fargo north dakota\\ Gold Answer: 120,762\\ Model Prediction: The population of Fargo, North Dakota \\ is about 120,000.\\ 
%   \\ Question: who ran the fastest 40 time in nfl history\\ Gold Answer: \textcolor{blue}{Bo Jackson}\\ Model Prediction: The fastest 40 yard dash in NFL history \\ was run by \textcolor{red}{Vincent Edward "Bo" Jackson}.\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Unit\\ Conversion\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}TIME\\ MONEY\\ QUANTITY\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Question: how long is the movie son of god\\ Gold Answer: \textcolor{blue}{138 minutes}\\ Model Prediction: The movie Son of God is \textcolor{red}{2 hours} \\ \textcolor{red}{and 18 minutes} long.\\ \\ Question: How tall was Napoleon?\\ Gold Answer: \textcolor{blue}{168 cm}\\ Model Prediction: Napoleon was \textcolor{red}{1.68m} tall.\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Contextual\\Paraphrase\end{tabular} &
% \begin{tabular}[c]{@{}c@{}}Unknown\\Others\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Question: the pectoralis minor is located deep\\ to which muscle\\ Gold Answer: \textcolor{blue}{beneath the pectoralis major}\\ Model Prediction: \textcolor{red}{under the pectoralis major muscle}.\end{tabular} \\ \hline
% \end{tabular}%
% }
% \caption{Categorization of surface form types depending on the entity types. Based on these errors, we sample few-shot examples for each entity type.}
% \label{tab:error_case}
% \end{table}



==> table/error_stat.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\hline
        & \multicolumn{2}{c}{NQ}  & \multicolumn{2}{c}{TQ}  \\ \hline
        & Turn Wrong & Turn Right & Turn Wrong & Turn Right \\ \hline
FID     & 106        & 143        & 29         & 118        \\
GPT3.5  & 188        & 247        & 46         & 144        \\
ChatGPT & 141        & 298        & 36         & 153        \\
GPT4    & 132        & 293        & 26         & 157        \\
Newbing & 104        & 256        & 23         & 170        \\ \hline
\end{tabular}%
}
\caption{Turn Wrong indicates the number of cases where the initial evaluation aligned with human judgement but became incorrect following the answer-set expansion. Turn Right denotes the number of cases where the initial evaluation differed from human judgement but became correct after the answer-set expansion."}
\label{tab:error_stat}
\end{table}


==> table/format_case.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|l|c|l|}
\hline
Diversity &
  Entity type &
  \multicolumn{1}{c|}{Format types} &
  \multicolumn{1}{c|}{Examples} \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\\ \\ \\ \\ \\ \\ \\ \\ \\ High\end{tabular}} &
  \multirow{4}{*}{\begin{tabular}[l]{@{}l@{}}\\ \\ \\Numeric\\- TIME\\- MONEY\\- QUANTITY\\- PERCENT\\- CARDINAL\\- DATE\\- ORDINAL\end{tabular}} &
  Numerals &
  \begin{tabular}[c]{@{}l@{}}Question: how many episodes are in\\ season 2 of the handmades tale\\ Gold Answer: \textcolor{blue}{13}\\ Model Prediction: The Season 2 of the\\ Handmaid's Tale have \textcolor{red}{thirteen} episodes.\end{tabular} \\ \cline{3-4} 
 &
   &
  \begin{tabular}[c]{@{}c@{}}Different\\ representation\\ (symbols,\\ abbreviation,\\ order)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Question: when was ye rishta kya kehlata \\ hai started\\ Gold Answer: \textcolor{blue}{January 12, 2009}\\ Model Prediction: The Ye Rishta Kya \\ Kehlata Hai started in \textcolor{red}{12 Jan., 2009}.\end{tabular} \\ \cline{3-4} 
 &
   &
  Specificity &
  \begin{tabular}[c]{@{}l@{}}Question: what's the population of fargo\\ north dakota\\ Gold Answer: \textcolor{blue}{120,762}\\ Model Prediction: The population of\\ Fargo, North Dakota is \textcolor{red}{about 120,000}.\end{tabular} \\ \cline{3-4} 
 &
   &
  \begin{tabular}[c]{@{}c@{}}Unit \\ conversion\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Question: how long is the movie son of god\\ Gold Answer: \textcolor{blue}{138 minutes}\\ Model Prediction: The movie Son of God is\\  \textcolor{red}{2 hours and 18 minutes} long.\end{tabular} \\ \cline{2-4} 
 &
  N/A &
  \begin{tabular}[c]{@{}l@{}}Contextual\\ paraphrase\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Question: the pectoralis minor is located deep\\  to which muscle\\ Gold Answer: \textcolor{blue}{beneath the pectoralis major}\\ Model Prediction: \textcolor{red}{under the pectoralis} \\ \textcolor{red}{major muscle}\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ \\ Med\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Non-numeric\\- PERSON\\- GPE\\- ORG\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Different\\ representation\\ (symbols,\\ abbreviation,\\ order)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Question: where was the ncaa football\\ championship game played 2018\\ Gold Answer: \textcolor{blue}{Atlanta, Georgia}\\ Model Prediction: The 2018 NCAA Football\\ Championship Game was played in \textcolor{red}{Atlanta, GA}.\end{tabular} \\ \cline{3-4} 
 &
   &
  Specificity &
  \begin{tabular}[c]{@{}l@{}}Question: who ran the fastest 40 time in nfl history\\ Gold Answer: \textcolor{blue}{Bo Jackson}\\ Model Prediction: The fastest 40 yard dash in NFL\\  history was run by \textcolor{red}{Vincent Edward "Bo" Jackson}.\end{tabular} \\ \hline
Low &
  \begin{tabular}[c]{@{}l@{}}Others\\ - NORP\\- FAC, LOC\\- etc.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Single\\ representation\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Question: what is the prison island in \\san francisco bay\\ Gold Answer: \textcolor{blue}{Alcatraz Island}\\ Model Prediction: \textcolor{red}{Alcatraz Island}\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Categorization of surface form types depending on the entity types. Based on these surface forms, we sample a few-shot examples for each entity type.}
\label{tab:format_case}
\end{table}
